ColorEdit: Training-free Image-Guided Color editing with diffusion model

Text-to-image (T2I) diffusion models, with their impressive generative capabilities, have been adopted for image editing tasks, demonstrating remarkable efficacy. However, due to attention leakage and collision between the cross-attention map of the object and the new color attribute from the text prompt, text-guided image editing methods may fail to change the color of an object, resulting in a misalignment between the resulting image and the text prompt. In this paper, we conduct an in-depth analysis on the process of text-guided image synthesizing and what semantic information different cross-attention blocks have learned. We observe that the visual representation of an object is determined in the up-block of the diffusion model in the early stage of the denoising process, and color adjustment can be achieved through value matrices alignment in the cross-attention layer. Based on our findings, we propose a straightforward, yet stable, and effective image-guided method to modify the color of an object without requiring any additional fine-tuning or training. Lastly, we present a benchmark dataset called COLORBENCH, the first benchmark to evaluate the performance of color change methods. Extensive experiments validate the effectiveness of our method in object-level color editing and surpass the performance of popular text-guided image editing approaches in both synthesized and real images.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.03.  Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/supplymentary.tex <==
\clearpage
%\setcounter{page}{1}
\maketitlesupplementary



\label{sec:supplymentary}
The Supplementary material of this paper consists of several sections that provide additional information and support for the main content.

\section{Additional information for Method Section}

\textbf{7.1 Framework pipeline and pseudocode for editing generated and real image} 

Algorithm ~\ref{alg: ALG1} and algorithm \ref{alg: ALG2} describe the pseudocode for editing generated and real images, respectively. We use Null-text Inversion \cite{mokady2023null} as the image inversion method to extract the value matrices of the reference color image $I^c$ and the latent space representation of the reference color image $I^c$ and the real image. 

\begin{algorithm}[!h]
\caption{Object-level Color Editing Algorithm for a generated image}
\label{alg: ALG1}

    \begin{flushleft}
        \hspace{0cm}  \textbf{Input:}: A source prompt $P$,  an interesting subject $O$ , a reference color image $I^c$\\
        \hspace{0cm}  \textbf{Output:}  A edited image $I^{T}$  \\
    \end{flushleft}
    
    \begin{algorithmic}[1]
        \State $z^{s}_T \in N (0, 1)$, a unit Gaussian random value sampled with random seed
       \State   $\{z^{s}_t\}^T_{t=0} , M^{S}_{cross}, M^{S}_{self}  \gets \text{DM}(z^{s}_T, P)$
        \State $Mask_{obj} \gets SAM(M^{S}_{cross}, O,   Generate(z^{S}_0)$
        \State $z^c_T \gets NullText - inv(I^c)$
        \State $V^c \gets LDM(z^c_T )$  $\triangleright$ with additional register forward hook method
             
        \For {$i = 1$ to $n$} 
            \State $z^{T}_T =  (1 \text{-} Mask_{obj} ) * z^{s}_{T} \text{+} Mask_{obj} * (z^{s}_T * (1 - ratio) \text{+}  z^c_T * ratio) $
            \For {$t = T, T-1, ..., 1$}           
                \If {$t > \tau $}
                    \State $z^{T}_{t-1} = \text{VAlignDM}(z^{T}_t, P, t, V^c) \{M^{T}_{self} \gets M^{S}_{self}\}$
                \Else
                    \State $z^{T}_{t-1} = \text{DM}(z^{T}_t, P, t) \{M^{T}_{self} \gets M^{S}_{self}\} $  
                \EndIf
    
                \If {$t < T-N $}
                    \State $z^{T}_{t-1}= (1 \text{-} Mask_{obj} ) * z^{s}_{t-1} \text{+} Mask_{obj} * z^{T}_{t-1} $
                 \EndIf
            \EndFor
        \State $I^{T}\gets Generate(z^{T}_0)$ 
        \State $z^{T}_T \gets NullText - Inv(I^{T}, P)$
        \EndFor
      
        \State \Return $I^{T}$
    
    \end{algorithmic}
\end{algorithm}


\begin{algorithm}[!h]
\caption{Object-level Color Editing Algorithm for a real image}
\label{alg: ALG2}

    \begin{flushleft}
        \hspace{0cm}  \textbf{input:}  A source image $I^{s}$, a text prompt $P$,  an interesting subject $O$ in the prompt $P$,  a reference color image $I^c$\\
        \hspace{0cm}  \textbf{Output:}  A edited image $I^{T}$  \\
    \end{flushleft}
    
    \begin{algorithmic}[1]
        \State $\{z^{s}_t\}^T_{t=0}, M^{S}_{cross}, M^{S}_{self} \gets NullText - inv(I^{s}, P)$
        \State $Mask_{obj} \gets SAM(M^{S}_{cross}, O, I^{s})$
        \State $z^c_T \gets NullText - inv(I^c)$
        \State $V^c \gets LDM(z^c_T )$  $\triangleright$ with additional register forward hook method
                     
        \For {$i = 1$ to $n$} 
          \State $z^{T}_T =  (1 \text{-} Mask_{obj} ) * z^{s}_{T} \text{+} Mask_{obj} * (z^{s}_T * (1 - ratio) \text{+}  z^c_T * ratio) $
          \For {$t = T, T-1, ..., 1$}
                \If {$t > \tau $}
                    \State $z^{T}_{t-1} = \text{VAlignDM}(z^{T}_t, P, t, V^c) \{M^{T}_{self} \gets M^{S}_{self}\}$
                \Else
                    \State $z^{T}_{t-1} = \text{DM}(z^{T}_t, P, t) \{M^{T}_{self} \gets M^{S}_{self}\} $  
                \EndIf
                
                 \If {$t < T-N $}
                    \State $z^{T}_{t-1}= (1 \text{-} Mask_{obj} ) * z^{s}_{t-1} \text{+} Mask_{obj} * z^{T}_{t-1} $
                 \EndIf
                 
            \EndFor
        \State $I_{T} \gets Generate(z^{T}_0)$ 
        \State $z^{T}_T \gets NullText - Inv(I^{T}, P)$
        \EndFor
    
        \State \Return $I^{T} $
    
    \end{algorithmic}
\end{algorithm}

\textbf{7.2 Cross-attention map in different blocks of U-Net} 

Fig.~\ref{fig:cross-attention-map-of-object-different-block} 
visualizes the average cross-attention maps of various objects from different blocks across all time steps. The cross-attention maps from different blocks are resized to the same resolution (512×512). As observed, the U-Net encoder captures some structural information of the object, but it is blurred (see the attention map of the 2nd and 3rd CrossAttnDownBlocks). In contrast, the U-Net decoder provides a clearer representation of the object's shape, contour, and texture. Specifically, the 1st, 2nd, and 3rd CrossAttnUpBlocks of the U-Net reveal progressively clearer shape, contour, and texture, respectively.  

\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{samples/figures/different_subject_cross_attention_map_different_block_v2.png}
    \caption{\textbf{Visualizing cross-attention map in the text-guided diffusion image generation.}  In this case, the text prompt is "a photo of *", where "*" represents a specific object. }    \label{fig:cross-attention-map-of-object-different-block}
\end{figure*}

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{samples/figures/instructPix2Pix_cross_attention_map_object_color.png}
    \caption{\textbf{Visualization of the Cross-attention maps for object and color attributes using InstructPix2Pix to edit the color. } In this example, the source image is generated with the prompt "an image of a toaster", while the edit text prompt is "turn the color of toaster to *," where "*" represents a specific color.} 
    \label{fig:instructPix2Pix_cross_attention_map_object_color}
\end{figure}
\textbf{7.3  Cross-attention leakage in training-based text-guided image editing methods} 

For training-based text-guided image editing methods \cite{brooks2023instructpix2pix, geng2024instructdiffusion, fu2023guiding}, the color change task is performed directly through text prompts, and the phenomenon of attention leakage also exists. As demonstrated in Fig.~\ref{fig:instructPix2Pix_cross_attention_map_object_color}, when the cross-attention map of the color attribute is distributed to the background of the image, the background color changes (e.g. when attempting to change the color of the toaster to white, gray, or green). 


\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{samples/figures/color_attribute_alignment_in_cross_layer.png}
    \caption{\textbf{Color attribute alignment in the cross-attention layer.}  The color of the object in the target image attends to the reference color image by applying AdaIN over its Value matrices $V^T$ using the Value matrices $V^c$ from the reference color image.  } 
    \label{fig:color_attribute_alignment_in_cross_layer}
\end{figure}

\textbf{7.4  color attribute alignment Pipeline} 

Fig.~\ref{fig:color_attribute_alignment_in_cross_layer} shows the color attribute alignment pipeline, color modification is achieved by utilizing the Value matrices of a reference image to normalize the Value matrices of the target image.

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{samples/figures/subject_mask_with_cross_attention_map_1.png}
    \caption{\textbf{Visualization of the edited image using P2P with the ground-truth mask.} As demonstrated, utilizing cross-attention maps to extract the binary mask of an object does not perfectly segment the object from the background, resulting in changes along the object's edges. In this example, the text prompt is "a photo of rabbit," and the target image, from left to right, shows the rabbit's color changing to white, black, and blue.} 
    \label{fig:subject_mask_with_cross_attention_map}
\end{figure}

\textbf{7.5 Object Mask generation and selection} 

In P2P\cite{hertz2022prompt} and MasaCtrl \cite{cao2023masactrl}, the binary mask was extracted directly from the cross-attention maps of the subject with a resolution of $16 \times 16$, which is obtained from the 3rd CrossAttnDownBlock and the 1st CrossAttnUpBlock in the U-Net. These cross-attention maps were then averaged and compared with a fixed threshold to generate the binary mask.  As seen in Fig.~\ref{fig:cross-attention-map-of-object-different-block}, the edges of the cross-attention maps in the 3rd CrossAttnDownBlock are blurred, leading to a binary mask that does not always precisely segment the object, especially around its edges, which resulting in changes along the object's edges ( see the example in Fig.~\ref{fig:subject_mask_with_cross_attention_map}, when we try to change the color of the rabbit to blue).

SAM \cite{kirillov2023segment} requires a segmentation prompt (e.g., point prompt) as input and generates a series of object masks $\{Mask_{obj}\}_n$. The point prompt (subject centroid) can be calculated from the cross-attention mask  $Mask^{cross}_{obj}$, which is obtained from the 1st CrossAttnUpBlock of the U-Net. To select the best object $Mask_{obj}$, we calculate a series of scores and choose the mask with $arg \space min_ns(i, n)$:
\[
s(i, n) = abs(1 - \frac{sum(Mask^{cross}_{obj})}{sum(Mask^{i}_{obj})} )
\]
where $sum(Mask)$ represents the area of zero value of the cross-attention mask or the mask generated from SAM. 
\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{samples/figures/qualitative_comparision_with_other_method_pikachu.png}
    \caption{\textbf{Comparisons to text-guided editing methods for generated image.} In each row, we present the modified image reflecting the desired color for the object using various methods. From top to bottom, the desired colors are "white," "gray," "black," "red," "yellow," "blue" and "green. In this case, the text prompt is "A photo of pikachu" and the object is "pikachu".
  } 
    \label{fig:color_editing_comparison_geneartion_image_all_color}
\end{figure*} 

\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{samples/figures/qualitative_comparision_with_other_method_real_image_v1.png}
    \caption{\textbf{Comparisons to text-guided editing methods for real images.} In each row, we present the modified image reflecting the desired color for the object using various methods. From top to bottom, the desired colors are "white," "gray," "black," "red," "yellow," "blue" and "green.
  } 
    \label{fig:color_editing_comparison_real_image_all_color}
\end{figure*}


\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{samples/figures/visualing_result_across_various_object_v2.png}
    \caption{\textbf{Color editing for generated images.} The first row displays the source image, while the subsequent rows depict the modified image with the desired color.} 
    \label{fig:colorEditGenerateImage}
\end{figure*}



\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{samples/figures/colorEditrealImage.png}
    \caption{\textbf{Color editing for real images.} The first row displays the source image, while the subsequent rows depict the modified image with the desired color.} 
    \label{fig:colorEditrealImage}
\end{figure*}



\section{Additional information for Experiment Section}

\textbf{8.1 Qualitative Experiments} 

For symthesised images, we compare our method with text-guided image editing methods InstructPix2Pix \cite{brooks2023instructpix2pix}, Instructdiffusion \cite{geng2024instructdiffusion},  MGIE \cite{fu2023guiding} , P2P \cite{hertz2022prompt}, PnP \cite{tumanyan2023plug} and FreePromptEditing \cite{liu2024towards}. For training-based methods InstructPix2Pix \cite{brooks2023instructpix2pix}, Instructdiffusion \cite{geng2024instructdiffusion} and MGIE \cite{fu2023guiding}, the prompt is "turn the color of the pikachu to $*$" and $*$ represents the specified color. For fine-tuning free approaches, P2P \cite{hertz2022prompt}, PnP \cite{tumanyan2023plug}, and FreePromptEditing \cite{liu2024towards}, the target prompt is "a photo of * pikachu", where "*" is the specific color.  Fig.~\ref{fig:color_editing_comparison_geneartion_image_all_color} provides all the color change outcomes for the generated image, including white, gray, black, red, yellow, blue, and green.

For real images, we conduct a comparison of our method with the text-guided image editing method InstructPix2Pix \cite{brooks2023instructpix2pix}, Instructdiffusion \cite{geng2024instructdiffusion},   MGIE \cite{fu2023guiding},  P2P \cite{hertz2022prompt}, PnP \cite{tumanyan2023plug} and FreePromptEditing \cite{liu2024towards}.  Since P2P cannot edit the real image, we use the Null text inversion \cite{mokady2023null} method to inverse the real image to its latent variable and then use P2P to change the color of the object.  Fig.~\ref{fig:color_editing_comparison_real_image_all_color} provides all the color change results for real images, including white, gray, black, red, yellow, blue, and green.

Fig.~\ref{fig:colorEditGenerateImage}  and Fig.~\ref{fig:colorEditrealImage} show the result of the generated image and the real image of various objects and image domains, including fruit, bird, insect, furry doll, plant, food, animal, toy, etc. Notice the color change of the object and the preserved background of the source image.  

\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{samples/figures/colorBenchSample.png}
    \caption{\textbf{Example data of COLORBENCH.} The COLORBENCH dataset including 406 images from 100 subjects, and the color of object in each image are change to 7 different colors, including white, gray, black, red, yellow, blue, and green.} 
    \label{fig:colorBenchSample}
\end{figure*}


\textbf{8.2 Data collection for Quantitative Experiments} 

For the generated dataset, the category of the 160 subjects includes fruits, vegetables, animals, insects, birds, musical instruments, furniture, electronic products, clothing, food, vehicles and cartoon characters. The list of the subjects are bread, hedgehog, raccoon, van, panda, pitcher, baseball, Pikachu, perch, helmet, butterfly, spinach, sofa, kale, onion, tarantula, minivan, chinchilla, Charmander, chair, soap, sunglasses, dolphin, porcupine, hippopotamus, kinkajou, ant, pineapple, hamburger, bulb, honeydew, fox, piranha, bison, donut, finch, lizard, Rilakkuma, waffle, cattle, mushroom, bagel, bench, python, tomato, tie, boots, leek, bongo, giraffe, bed, bow, hovercraft, scooter, wolf, bee, egg, sweater, dog, cymbal, lettuce, starfish, sparrow, starfruit, celery, turtle, isopod, lime, humidifier, parrot, ladle, armadillo, monkey, avocado, snake, skunk, bird, toaster, rat, koala, camel, apricot, tank, apple, hoodie, squirrel, lemon, tiger, cantaloupe, weasel, sheep, rabbit, snail, elephant, bear, Pichu, hamster, goldfish, coat, shorts, ladybug, lion, ball, gun, SUV, otter, tick, table, beaver, mackerel, gerbil, handbag, artichoke, asparagus, cake, cauliflower, speaker, ocelot, banana, backpack, broccoli, Cubone, lemur, scorpion, javelina, canoe, timpani, dragonfly, cup, pumpkin, coconut, iguana, lobster, orange, snowman, deer, parsnip, peach, limousine, pear, purse, ferret, antelope, spoon, lamp, pillow, carrot, cabbage, truck, frog, grapefruit, drum, brownie, moose, Simba, scarf, mango, glider, cello.  The text templates we use to generate the prompt are: 1) "a photo of a \{\}", 2) "an image of a \{\}" , 3) "a photo of a nice \{\}", 4) "a photo of a large \{\}", 5) "a good photo of a \{\}", 6) "a rendition of a \{\}", and 7) "a toy of a \{\}". For quantitative analysis, we generated a dataset comprising 1,120 image-prompt pairs, with the source images created with random seed.  

For real image dataset, the dataset includes 406 images from 100 subjects, which include: apple, cat, dinosaur, garlic, ladybug, peach, strawberry, asparagus, celery, dog, glove, leaf, peanut, sugar, avocado, champagne, doughnut, goldfish, lemon, pear, suitcase, backpack, cherry, dragon, giraffe, lion, pigeon, tomato, banana, chick, dragonfly, grape, macaron, potato,  T-shirt,  bee,  chili,  eagle,  hamburger,  mango, raspberry,  bird,  chiwawa,  earthworm, handbag, mantis, rhino, vegetable, blueberry, coat, eggplant, hat,  mushroom,  rock, walnut,  boots, cocktail, elephant,   heel,  noodle, sausage, wasp, bug, coconut, fig,   hornet, nut, scorpion, watermelon, butter, cookie, fish, horse, okra, Shells, yam, butterfly, cricket, flea, icecream, orange, shirt, cantaloupe, Croton, flower, insect, pancake, shoe, cap, cucumber, fly, kiwifruit, parrot, spider, car, daikon, fruit, ladybird, pea, spinach. An example of COLORBENCH is given in Fig.~\ref{fig:colorBenchSample} .


\textbf{8.3 Evaluation Metrics for Quantitative Experiments} 

For evaluation metrics, we measure semantic similarity using the DINO score \cite{caron2021emerging}, which is designed to assess how similar two images are in terms of their semantic content, including objects, scenes, and concepts. However, to eliminate the effect of the object's color on the DINO score, we compute the DINO score using the grayscale versions of both the source and target images and call it $DS$.  For structural similarity, we applied SSIM \cite{wang2004image}, which evaluates the similarity between two images based on luminance, contrast, and structure at the pixel level.   To verify that the edited image contains the specified color of the object, we calculate the CLIP Score (CLIP cosine similarity) \cite{radford2021learning} between the image and its corresponding text description. For instance, if the source image is generated with the prompt "a photo of a squirrel" and the color of the squirrel is altered to red, the CLIP cosine similarity is computed between the edited image and the text description "a photo of a red squirrel". A higher CLIP score (CS) indicates that the image and text are semantically aligned, which means that the image accurately depicts the content described by the text.  Although the CLIP score effectively measures semantic alignment, it does not directly evaluate other critical aspects of image quality, such as texture, color accuracy, or structural fidelity. To assess color accuracy, we calculate the L1 loss between the target image and the corresponding pure color image within the object area using the HSV color system, since the HSV color system provides a more human-friendly way of manipulating colors compared to the RGB model, which we call $L1^{HSV}_{obj}$.  To eliminate the influence of color purity and lightness, we exclude the saturation and value components and calculate the L1 loss based solely on the hue, which we call the loss L1 of Hue of the object $L1^{Hue}_{obj}$. A lower L1 loss signifies a closer alignment between the object and the desired target color hue. To quantify the preservation of background information, we employ the object's mask to isolate the background in both the source and target images, subsequently evaluating the similarity using LPIPS \cite{zhang2018unreasonable} and call it $LPIPS_{bg}$.  A lower LPIPS value indicates better preservation of background information. 

For color accuracy measure, the RGB values we use to construct the pure color image are: 1) black: (0, 0, 0), 2) white: (255, 255, 255), 3) gray: (128, 128, 128), 4) red: (255, 0, 0), 5) yellow: (255, 255, 0), 6) blue: (0, 0, 255), 7) green: (0, 255, 0). 


\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{samples/figures/human_evaluation_example.png}
\caption{\textbf{Screenshot from the Human Evaluation.} The second row of the image shows the results obtained by different methods. The user is asked to rank the performance of each method from 0 to 5. 0 means the worst,while 5 means the best. }
  
    \label{fig:human_evaluation_example}
\end{figure*}

\begin{table*}
    \centering
  \begin{tabular}{ccccccc}
    \toprule
    & $DS\uparrow$&$SSIM\uparrow$&   $CS\uparrow$&$L1^{Hue}_{obj} \downarrow$& $L1^{HSV}_{obj} \downarrow$&$LPIPS_{bg} \downarrow$\\
    \midrule
    w/o cross-attn. Alignment&  \textbf{0.965}& \textbf{0.875}&  17.766 &52.677 & 59.509 &\textbf{0.007}\\
 First 20\% time step
(our)& 0.957 & 0.830 & 17.906 & \textbf{50.800}& 56.655 &0.016 
\\
 First 50\% time step& 0.876 & 0.715 & \textbf{17.955}& 50.864 & \textbf{55.944}&0.032 
\\
    All time step& 0.622 & 0.622 &   17.943 &52.084 & 55.962 &0.046 
\\
      \bottomrule
\end{tabular}
  \caption{\textbf{Quantitative evaluation results with cross-attention value alignment in different diffusion time step.} The reference color image blending ratio is set to 0.1}
  \label{tab:t4}
\end{table*}

\textbf{8.4 Quantitative evaluation results for Cross-attention value Alignment} 

 Table \ref{tab:t4} shows that without alignment of cross-attention values, the structures of the object remain well preserved. However, as cross-attention values are aligned during further denoising steps, the object's structural integrity progressively deteriorates (see how $DS$ and $SSIM$ change through different cross-attention value alignment plans). For the color change of the object, the effect improves as the number of alignment steps of values increases. However, it decreases when the alignment of the cross-attention value is applied throughout the entire denoising process (see how $L1^{Hue}_{obj}$ and $L1^{HSV}_{obj}$ change in the table).


\begin{table*}
    \centering
  \begin{tabular}{ccccccc}
    \toprule
    Ratio& $DS\uparrow$&$SSIM\uparrow$&   $CS\uparrow$&$L1^{Hue}_{obj} \downarrow$& $L1^{HSV}_{obj} \downarrow$&$LPIPS_{bg} \downarrow$\\
    \midrule
    0.0&  0.916 & 0.783 &  17.726&50.768& 57.435 &0.018 \\
 0.05& 0.948 & 0.829 & 17.798 & 51.092 & 57.649 &\textbf{0.015}\\
 0.1& \textbf{0.957}& \textbf{0.830}& 17.906& 50.800& \textbf{56.655}&0.016\\
    0.15& 0.946 & 0.795 &   \textbf{17.925}&\textbf{50.721}& 56.935 &0.018 
\\
 0.2& 0.922 & 0.760 & 17.862 & 50.860 & 57.944 &0.020 
\\
      \bottomrule
\end{tabular}
  \caption{\textbf{Quantitative evaluation results  with different reference color image latent blending ratio.} The alignment of the attention value is performed in the first 20\% of the diffusion time step.} 
    \label{tab:t5}
\end{table*}

\textbf{8.5 Quantitative evaluation results for different reference color image blending ratio} 

 Table \ref{tab:t5} shows the quantitative evaluation result of different latent variable blending ratios of the reference color image. As shown in the table, setting the ratio to 0.1 results in the least structural distortion of the object. However, when the ratio is set to 0.15, the color change effect is optimal, though there is a slight loss in the object's structural integrity.

\textbf{8.6 Details of Human Evaluation} 

As described in the main paper, we randomly select 100 pairs of source and target images.  The distribution of desired color in target images is: 15 white, 14 gray, 13 black, 14 red, 15 yellow, 14 blue, and 15 green. The involved subjects include: cattle, celery, handbag, honeydew, onion, perch, waffle, drum, orange, pineapple, tomato, finch, spinach, artichoke, banana, cup, coconut, dragonfly, lizard, porcupine, egg, ferret, lime, wolf, fox, mushroom, snowman, pumpkin, bread, lettuce, ladybug, tarantula, lobster, Pichu, bench, bongo, butterfly, cello, coat, hoodie, melmet, isopod, baseball, pillow, dolphin, lion, tank, rat, speaker, kale, lemon, tiger, asparagus, Pikachu, grapefruit, javelina, sofa, starfruit, bagel, piranha, and apple.

The color editing effect of an object refers to how closely the object's color modification aligns with the target color. Object identity preservation measures the extent to which the object's original identity is retained in the edited image. The preservation of the background indicates how well the background remains intact without distortion. Overall editing quality encompasses the naturalness of the color modification, including the overall realism of the image post-editing.

The human evaluation format is provided in Fig.\ref{fig:human_evaluation_example}  where the user is asked to rank the performance of each method in the following aspects: 1) color editing of the object, 2) preservation of object identity, 3) preservation of background, and 4) overall editing quality. To prevent potential bias, we use "Method X" as a placeholder for the specific method.
